Chronax: A Jax Library for Forecasting and Conformal Inference

Time-series forecasting is central to many scientific and industrial domains, such as energy systems, climate modeling, finance, and retail. While forecasting methods have evolved from classical statistical models to automated, and neural approaches, the surrounding software ecosystem remains anchored to the traditional Python numerical stack. Existing libraries rely on interpreter-driven execution and object-oriented abstractions, limiting composability, large-scale parallelism, and integration with modern differentiable and accelerator-oriented workflows. Meanwhile, today's forecasting increasingly involves large collections of heterogeneous time series data, irregular covariates, and frequent retraining, placing new demands on scalability and execution efficiency. JAX offers an alternative paradigm to traditional stateful numerical computation frameworks based on pure functions and program transformations such as just-in-time compilation and automatic vectorization, enabling end-to-end optimization across CPUs, GPUs, and TPUs. However, this modern paradigm has not yet been fully incorporated into the design of forecasting systems. We introduce Chronax, a JAX-native time-series forecasting library that rethinks forecasting abstractions around functional purity, composable transformations, and accelerator-ready execution. By representing preprocessing, modeling, and multi-horizon prediction as pure JAX functions, Chronax enables scalable multi-series forecasting, model-agnostic conformal uncertainty quantification, and seamless integration with modern machine learning and scientific computing pipelines.

==> smlcrm-logo.tex <==
\def\smlcrm@wordmark@w{862.48}
\def\smlcrm@wordmark@h{190.14}
\def\smlcrm@wordmark@draw{%
  \fill (25.41,-59.90) -- (15.06,-54.52) -- (106.12,-0.00) -- (25.41,-59.90) -- cycle;
  \fill (67.82,-81.37) -- (54.62,-74.69) -- (148.00,-21.85) -- (67.82,-81.37) -- cycle;
  \fill (110.21,-102.83) -- (94.89,-95.07) -- (189.89,-43.69) -- (110.21,-102.83) -- cycle;
  \fill (164.48,-130.24) -- (174.82,-135.62) -- (83.77,-190.14) -- (164.48,-130.24) -- cycle;
  \fill (122.07,-108.78) -- (135.27,-115.46) -- (41.88,-168.29) -- (122.07,-108.78) -- cycle;
  \fill (79.67,-87.31) -- (95.00,-95.07) -- (0.00,-146.45) -- (79.67,-87.31) -- cycle;
  \fill (253.34,-128.73) .. controls (248.32,-128.73) and (243.53,-127.96) .. (238.95,-126.43) .. controls (234.37,-124.90) and (230.77,-122.90) .. (228.14,-120.46) -- (231.62,-113.13) .. controls (234.13,-115.33) and (237.32,-117.14) .. (241.21,-118.58) .. controls (245.10,-120.02) and (249.14,-120.74) .. (253.34,-120.74) .. controls (257.16,-120.74) and (260.26,-120.30) .. (262.65,-119.42) .. controls (265.03,-118.54) and (266.79,-117.34) .. (267.91,-115.80) .. controls (269.03,-114.26) and (269.60,-112.53) .. (269.60,-110.58) .. controls (269.60,-108.32) and (268.86,-106.51) .. (267.39,-105.13) .. controls (265.92,-103.75) and (264.01,-102.64) .. (261.65,-101.79) .. controls (259.30,-100.94) and (256.71,-100.21) .. (253.89,-99.58) .. controls (251.07,-98.95) and (248.23,-98.22) .. (245.38,-97.37) .. controls (242.53,-96.52) and (239.93,-95.44) .. (237.58,-94.13) .. controls (235.23,-92.81) and (233.33,-91.04) .. (231.89,-88.82) .. controls (230.45,-86.60) and (229.73,-83.73) .. (229.73,-80.22) .. controls (229.73,-76.71) and (230.62,-73.72) .. (232.41,-70.86) .. controls (234.20,-68.01) and (236.95,-65.72) .. (240.68,-64.00) .. controls (244.41,-62.28) and (249.16,-61.41) .. (254.92,-61.41) .. controls (258.74,-61.41) and (262.54,-61.91) .. (266.30,-62.91) .. controls (270.06,-63.91) and (273.32,-65.36) .. (276.08,-67.24) -- (272.98,-74.76) .. controls (270.16,-72.88) and (267.18,-71.52) .. (264.05,-70.67) .. controls (260.91,-69.82) and (257.88,-69.40) .. (254.93,-69.40) .. controls (251.23,-69.40) and (248.19,-69.87) .. (245.81,-70.81) .. controls (243.43,-71.75) and (241.69,-73.00) .. (240.59,-74.57) .. controls (239.49,-76.14) and (238.94,-77.89) .. (238.94,-79.83) .. controls (238.94,-82.15) and (239.68,-84.00) .. (241.15,-85.38) .. controls (242.62,-86.76) and (244.54,-87.86) .. (246.89,-88.67) .. controls (249.24,-89.49) and (251.83,-90.22) .. (254.65,-90.88) .. controls (257.47,-91.54) and (260.31,-92.27) .. (263.16,-93.09) .. controls (266.01,-93.91) and (268.61,-94.97) .. (270.96,-96.29) .. controls (273.31,-97.61) and (275.21,-99.36) .. (276.65,-101.56) .. controls (278.09,-103.75) and (278.81,-106.57) .. (278.81,-110.02) .. controls (278.81,-113.47) and (277.90,-116.43) .. (276.08,-119.28) .. controls (274.26,-122.13) and (271.46,-124.42) .. (267.67,-126.14) .. controls (263.88,-127.87) and (259.10,-128.73) .. (253.33,-128.73) -- cycle;
  \fill (290.19,-127.98) -- (290.19,-62.16) -- (299.59,-62.16) -- (299.59,-127.97) -- (290.19,-127.97) -- cycle;
  \fill (313.66,-127.98) -- (313.66,-62.16) -- (321.37,-62.16) -- (350.89,-111.89) -- (346.75,-111.89) -- (375.89,-62.16) -- (383.60,-62.16) -- (383.69,-127.97) -- (374.66,-127.97) -- (374.57,-76.36) -- (376.73,-76.36) -- (350.78,-119.98) -- (346.46,-119.98) -- (320.32,-76.36) -- (322.67,-76.36) -- (322.67,-127.97) -- (313.64,-127.97) -- cycle;
  \fill (424.85,-128.73) .. controls (416.20,-128.73) and (409.40,-126.26) .. (404.45,-121.30) .. controls (399.50,-116.35) and (397.02,-109.11) .. (397.02,-99.58) -- (397.02,-62.16) -- (406.42,-62.16) -- (406.42,-99.20) .. controls (406.42,-106.53) and (408.03,-111.89) .. (411.26,-115.28) .. controls (414.49,-118.66) and (419.05,-120.36) .. (424.94,-120.36) .. controls (430.83,-120.36) and (435.48,-118.67) .. (438.71,-115.28) .. controls (441.94,-111.89) and (443.55,-106.54) .. (443.55,-99.20) -- (443.55,-62.16) -- (452.67,-62.16) -- (452.67,-99.58) .. controls (452.67,-109.11) and (450.21,-116.35) .. (445.29,-121.30) .. controls (440.37,-126.25) and (433.55,-128.73) .. (424.84,-128.73) -- cycle;
  \fill (466.09,-127.98) -- (466.09,-62.16) -- (475.49,-62.16) -- (475.49,-119.79) -- (511.12,-119.79) -- (511.12,-127.97) -- (466.09,-127.97) -- cycle;
  \fill (516.63,-127.98) -- (546.43,-62.17) -- (555.74,-62.17) -- (585.64,-127.98) -- (575.77,-127.98) -- (549.16,-67.43) -- (552.92,-67.43) -- (526.31,-127.98) -- (516.63,-127.98) -- cycle (529.32,-111.52) -- (531.86,-104.00) -- (568.90,-104.00) -- (571.63,-111.52) -- (529.32,-111.52) -- cycle;
  \fill (621.56,-128.73) .. controls (616.54,-128.73) and (611.92,-127.90) .. (607.69,-126.24) .. controls (603.46,-124.58) and (599.79,-122.23) .. (596.69,-119.19) .. controls (593.59,-116.15) and (591.16,-112.60) .. (589.40,-108.52) .. controls (587.64,-104.45) and (586.77,-99.96) .. (586.77,-95.08) .. controls (586.77,-90.20) and (587.65,-85.71) .. (589.40,-81.63) .. controls (591.15,-77.56) and (593.60,-74.00) .. (596.73,-70.96) .. controls (599.86,-67.92) and (603.55,-65.57) .. (607.78,-63.91) .. controls (612.01,-62.25) and (616.63,-61.42) .. (621.65,-61.42) .. controls (626.67,-61.42) and (631.41,-62.28) .. (635.71,-64.01) .. controls (640.00,-65.73) and (643.65,-68.29) .. (646.66,-71.67) -- (640.55,-77.59) .. controls (638.04,-74.96) and (635.22,-73.00) .. (632.09,-71.71) .. controls (628.96,-70.43) and (625.60,-69.78) .. (622.03,-69.78) .. controls (618.46,-69.78) and (614.90,-70.41) .. (611.74,-71.66) .. controls (608.57,-72.91) and (605.83,-74.67) .. (603.51,-76.92) .. controls (601.19,-79.18) and (599.39,-81.86) .. (598.10,-84.96) .. controls (596.82,-88.06) and (596.17,-91.43) .. (596.17,-95.07) .. controls (596.17,-98.71) and (596.81,-102.07) .. (598.10,-105.18) .. controls (599.38,-108.28) and (601.19,-110.96) .. (603.51,-113.22) .. controls (605.83,-115.48) and (608.57,-117.23) .. (611.74,-118.48) .. controls (614.90,-119.74) and (618.33,-120.36) .. (622.03,-120.36) .. controls (625.73,-120.36) and (628.96,-119.72) .. (632.09,-118.43) .. controls (635.22,-117.15) and (638.04,-115.16) .. (640.55,-112.46) -- (646.66,-118.38) .. controls (643.65,-121.77) and (640.00,-124.34) .. (635.71,-126.09) .. controls (631.41,-127.85) and (626.70,-128.72) .. (621.56,-128.72) -- cycle;
  \fill (657.75,-127.98) -- (657.75,-62.16) -- (683.42,-62.16) .. controls (689.18,-62.16) and (694.10,-63.07) .. (698.18,-64.89) .. controls (702.25,-66.71) and (705.39,-69.34) .. (707.58,-72.79) .. controls (709.77,-76.24) and (710.87,-80.34) .. (710.87,-85.10) .. controls (710.87,-89.86) and (709.77,-93.95) .. (707.58,-97.37) .. controls (705.39,-100.79) and (702.25,-103.40) .. (698.18,-105.22) .. controls (694.10,-107.04) and (689.18,-107.95) .. (683.42,-107.95) -- (662.92,-107.95) -- (667.15,-103.62) -- (667.15,-127.97) -- (657.75,-127.97) -- cycle (667.15,-104.57) -- (662.92,-99.96) -- (683.13,-99.96) .. controls (689.15,-99.96) and (693.71,-98.66) .. (696.81,-96.06) .. controls (699.91,-93.46) and (701.46,-89.81) .. (701.46,-85.11) .. controls (701.46,-80.41) and (699.91,-76.78) .. (696.81,-74.20) .. controls (693.71,-71.63) and (689.15,-70.35) .. (683.13,-70.35) -- (662.92,-70.35) -- (667.15,-65.65) -- (667.15,-104.57) -- cycle (701.75,-127.98) -- (685.02,-104.10) -- (695.08,-104.10) -- (712.00,-127.98) -- (701.75,-127.98) -- cycle;
  \fill (751.01,-128.73) .. controls (742.36,-128.73) and (735.56,-126.26) .. (730.61,-121.30) .. controls (725.66,-116.35) and (723.18,-109.11) .. (723.18,-99.58) -- (723.18,-62.16) -- (732.58,-62.16) -- (732.58,-99.20) .. controls (732.58,-106.53) and (734.19,-111.89) .. (737.42,-115.28) .. controls (740.65,-118.66) and (745.21,-120.36) .. (751.10,-120.36) .. controls (756.99,-120.36) and (761.64,-118.67) .. (764.87,-115.28) .. controls (768.10,-111.89) and (769.71,-106.54) .. (769.71,-99.20) -- (769.71,-62.16) -- (778.83,-62.16) -- (778.83,-99.58) .. controls (778.83,-109.11) and (776.37,-116.35) .. (771.45,-121.30) .. controls (766.53,-126.25) and (759.71,-128.73) .. (751.00,-128.73) -- cycle;
  \fill (792.43,-127.98) -- (792.43,-62.16) -- (800.14,-62.16) -- (829.66,-111.89) -- (825.52,-111.89) -- (854.66,-62.16) -- (862.37,-62.16) -- (862.46,-127.97) -- (853.43,-127.97) -- (853.34,-76.36) -- (855.50,-76.36) -- (829.55,-119.98) -- (825.23,-119.98) -- (799.09,-76.36) -- (801.44,-76.36) -- (801.44,-127.97) -- (792.41,-127.97) -- cycle;
}
\def\smlcrm@emblem@w{531.22}
\def\smlcrm@emblem@h{531.93}
\def\smlcrm@emblem@draw{%
  \fill (71.08,-167.57) -- (42.14,-152.52) -- (296.87,-0.00) -- (71.08,-167.57) -- cycle;
  \fill (189.72,-227.62) -- (152.80,-208.94) -- (414.04,-61.12) -- (189.72,-227.62) -- cycle;
  \fill (308.32,-287.67) -- (265.45,-265.96) -- (531.22,-122.23) -- (308.32,-287.67) -- cycle;
  \fill (460.14,-364.37) -- (489.08,-379.41) -- (234.35,-531.93) -- (460.14,-364.37) -- cycle;
  \fill (341.50,-304.31) -- (378.41,-323.00) -- (117.17,-470.81) -- (341.50,-304.31) -- cycle;
  \fill (222.89,-244.27) -- (265.76,-265.97) -- (0.00,-409.70) -- (222.89,-244.27) -- cycle;
}

